Reward Reports for Reinforcement Learning

Building systems that are good for society in the face of complex societal effects requires a dynamic approach. Recent approaches to machine learning (ML) documentation have demonstrated the promise of discursive frameworks for deliberation about these complexities. However, these developments have been grounded in a static ML paradigm, leaving the role of feedback and post-deployment performance unexamined. Meanwhile, recent work in reinforcement learning has shown that the effects of feedback and optimization objectives on system behavior can be wide-ranging and unpredictable. In this paper we sketch a framework for documenting deployed and iteratively updated learning systems, which we call Reward Reports. Taking inspiration from various contributions to the technical literature on reinforcement learning, we outline Reward Reports as living documents that track updates to design choices and assumptions behind what a particular automated system is optimizing for. They are intended to track dynamic phenomena arising from system deployment, rather than merely static properties of models or data. After presenting the elements of a Reward Report, we discuss a concrete example: Meta's BlenderBot 3 chatbot. Several others for game-playing (DeepMind's MuZero), content recommendation (MovieLens), and traffic control (Project Flow) are included in the appendix.

==> reward-report-questions.tex <==


\newcommand{\descr}{\small \emph}
\newcommand{\eg}{\textit{e.g.}}             % For example
\newcommand{\etc}{\textit{etc}.}           % So on...
\newcommand{\ie}{\textit{i.e.}}             % literally


\newcommand{\SystemDetails}[4]{
\section{System Details}
\subsection{System Owner}
\descr{This may be the designer deploying the system, a larger agency or body, or some combination of the two. The entity completing the report should also be indicated.}

#1
% % % % % 
\subsection{Dates}
\descr{The
known or intended timespan over which this reward function \& optimization is active. }

#2
% % % % % 
\subsection{Feedback \& Communication}
\descr{Contact information for the designer, team, or larger agency responsible for system deployment.}

#3
% % % % % 
\subsection{Other Resources}
\descr{Where can users or stakeholders find more information about this system? Is this system based on one or more research
papers?}

#4
}

% % % % % % % % % % 
\newcommand{\OptIntent}[4]{
\section{Optimization Intent}
\subsection{Goal of Reinforcement}
\descr{A statement of system scope and purpose, including the planning horizon and justification of
a data-driven approach to policy design (\eg{} the use of reinforcement learning or repeated retraining). This justification
should contrast with alternative approaches, like static models and hand-designed policies. What is there to gain with
the chosen approach?}

#1
% % % % % 
\subsection{Defined Performance Metrics}
\descr{A list of “performance metrics” included explicitly in the reward
signal, the criteria for why these metrics were chosen, and from where these criteria were drawn (\eg{} government
agencies, domain precedent, GitHub repositories, toy environments). Performance metrics that are used by the designer
to tune the system, but not explicitly included in the reward signal should also be reported here.}

#2
% % % % % 
\subsection{Oversight Metrics}
\descr{Are there any additional metrics not included in the reward signal but relevant for vendor or system oversight (e.g.
performance differences across demographic groups)? Why aren’t they part of the reward signal, and why must they
be monitored? }

#3
% % % % % 
\subsection{Known Failure Modes}
\descr{A description of any prior known instances of “reward hacking” or model
misalignment in the domain at stake, and description of how the current system avoids this.}


#4
}

% % % % % % % % % % 
\newcommand{\Interfaces}[4]{
\section{Institutional Interface}
\subsection{Deployment Agency}
\descr{ What other agency or controlling entity roles, if any, are intended to be subsumed by the
system? How may these roles change following system deployment?}

#1
% % % % % 
\subsection{Stakeholders}
\descr{What other interests are implicated in the design specification or system deployment, beyond the designer? What role will these interests play in
subsequent report documentation? What other entities, if any, does the deployed system interface with whose interests
are not intended to be in scope? }

#2
% % % % % 
\subsection{Explainability \& Transparency}
\descr{Does the system offer explanations of its decisions
or actions? What is the purpose of these explanations? To what extent is the policy transparent, \ie{} can decisions or
actions be understood in terms of meaningful intermediate quantities? }

#3
% % % % % 
\subsection{Recourse}
\descr{Can stakeholders or users contest
the decisions or actions of the system? What processes, technical or otherwise, are in place to handle this?}

#4
}

% % % % % % % % % % 
\newcommand{\Implementation}[7]{
\section{Implementation}
\subsection{Reward Details}
\descr{How was the reward function engineered? Is it
based on a well-defined metric? Is it tuned to represent a specific behavior? Are multiple terms scaled to make one
central loss, and how was the scaling decided?}

#1
% % % % % 
\subsection{Environment Details}
\descr{Description of states, observations, and actions
with reference to planning horizon and hypothesized dynamics/impact. What dynamics are brought into the scope of
the optimization via feedback? Which dynamics are left external to the system, as drift? Have there been any observed
gaps between conceptualization and resultant dynamics?}



#2
% % % % % 
\subsection{Measurement Details}
\descr{How are the components of the
reward and observations measured? Are measurement techniques consistent across time and data sources? Under what
conditions are measurements valid and correct? What biases might arise during the measurement process? }

#3
% % % % % 
\subsection{Algorithmic Details}
\descr{The key points on the specific algorithm(s) used for learning and planning. This includes the form of the
policy (\eg{} neural network, optimization problem), the class of learning algorithm (\eg{} model-based RL, off-policy RL,
repeated retraining), the form of any intermediate model (\eg{} of the value function, dynamics function, reward function),
technical infrastructure, and any other considerations necessary for implementing the system. Is the algorithm publicly
documented and is code publicly available? Have different algorithms been used or tried to accomplish the same goal?}

#4
% % % % % 
\subsection{Data Flow}
\descr{How is data collected, stored, and used for (re)training? How frequently are various components of the
system retrained, and why was this frequency chosen? Could the data exhibit sampling bias, and is this accounted for in
the learning algorithm? Is data reweighted, filtered, or discarded? Have data sources changed over time?}

#5
% % % % % 
\subsection{Limitations}
\descr{Discussion and justification of modeling choices arising from computational, statistical, and measurement limitations.
How might (or how have) improvements in computational power and data collection change(d) these considerations
and impact(ed) system behavior?}

#6
% % % % % 
\subsection{Engineering Tricks}
\descr{RL systems are known to be sensitive to implementation tricks
that are key to performance. Are there any design elements that have a surprisingly strong impact on performance? For example,
state-action normalization, hard-coded curricula, model-initialization, loss bounds, or more?}

#7
}

% % % % % % % % % % 
\newcommand{\Evaluation}[4]{
\section{Evaluation}
\subsection{Evaluation Environment}
\descr{ How is the system evaluated (and if applicable, trained) prior to deployment (\eg{} using
simulation, static datasets, \etc{})? Exhaustive details of the offline evaluation environment should be provided. For simulation, details should
include description or external reference to the underlying model, ranges of parameters, etc. 
For evaluation on static datasets, considering referring to associated documentation (\eg{} \emph{Datasheets}~\cite{gebru2021datasheets}).
}

#1
% % % % % 
\subsection{Offline Evaluations}
\descr{Present and discuss the results of offline
evaluation. 
For static evaluation, consider referring to associated documentation (\eg{} \emph{Model Cards}~\cite{mitchell2019model}).
If applicable, compare the behaviors arising from counterfactual specifications
(e.g. of states, observations, actions). }

#2
% % % % % 
\subsection{Evaluation Validity}
\descr{ To what extent is it reasonable to draw conclusions about
the behavior of the deployed system based on presented offline evaluations? What is the current state of understanding
of the online performance of the system? If the system has been deployed, were any unexpected behaviors observed?}

#3
% % % % % 
\subsection{Performance standards}
\descr{What standards of performance and safety is the system required to meet? Where do these
standards come from? How is the system verified to meet these standards?}

#4

% \descr{Evaluation of simulated behaviors as well as exhaustive details on simulation parameters. This can include the timestep used in simulation, underlying world model, computational software used, external references,
% and any more relevant information. Was the model developed in a closed simulation? Are there plans for transferring
% from sim to real? Is the deployed environment exactly the same as the training environment?}


% \descr{Is the implementation centered around finding a solution or recreating a known solution to
% a problem? Has the environment been modified to make the task easier? Is there an existence of a predetermined
% "optimal" behavior?}

% \descr{The state of understanding the quantified performance of the initial agent used by the system.
% Were the observed behaviors expected?}
}

% % % % % % % % % % 
\newcommand{\Maintenance}[3]{
\section{System Maintenance}
\subsection{Reporting Cadence}
\descr{The intended
timeframe for revisiting the reward report. How was this decision reached and motivated? }

#1
% % % % % 
\subsection{Update Triggers}
\descr{Specific
events (projected or historic) significant enough to warrant revisiting this report, beyond the cadence outlined above.
Example triggers include a defined stakeholder group empowered to demand a system audit, or a specific metric (either
of performance or oversight) that falls outside a defined threshold of critical safety.}

#2
% % % % % 
\subsection{Changelog}
\descr{Descriptions of updates
and lessons learned from observing and maintaining the deployed system. This includes when the updates were made
and what motivated them in light of previous reports. The changelog comprises the central difference between reward
reports and other forms of machine learning documentation, as it directly reflects their intrinsically dynamic nature.}


#3


}
